A proximal Newton framework for composite minimization: Graph learning without Cholesky decompositions and matrix inversions

We propose an algorithmic framework for convex minimization problems of a composite function with two terms: a self-concordant function and a possibly nonsmooth regularization term. Our method is a new proximal Newton algorithm that features a local quadratic convergence rate. As a specific instance of our framework, we consider the sparse inverse covariance matrix estimation in graph learning problems. Via a careful dual formulation and a novel analytic step-size selection procedure, our approach for graph learning avoids Cholesky decompositions and matrix inversions in its iteration making it attractive for parallel and distributed implementations.

==> acknowledgements.tex <==
% \newline
% \vskip0.1cm
% \noindent\textbf{Acknowledgements. }
\section*{Acknowledgements}
This work was supported in part by the European Commission under Grant MIRG-268398, ERC Future Proof, and SNF 200021-132548. 
Volkan Cevher also would like to acknowledge Rice University for his Faculty Fellowship.
